Modeling Dense Star Clusters in the Milky Way and Beyond with the $\texttt{CMC}$ Cluster Catalog

We present a set of 148 independent $N$-body simulations of globular clusters (GCs) computed using the code $\texttt{CMC}$ ($\texttt{Cluster Monte Carlo}$). At an age of $\sim10-13\,$Gyr, the resulting models cover nearly the full range of cluster properties exhibited by the Milky Way GCs, including total mass, core and half-light radii, metallicity, and galactocentric distance. We use our models to investigate the role that stellar-mass black holes play in the process of core collapse. Furthermore, we study how dynamical interactions affect the formation and evolution of several important types of sources in GCs, including low-mass X-ray binaries, millisecond pulsars, blue stragglers, cataclysmic variables, Type Ia supernovae, calcium-rich transients, and merging compact binaries. While our focus here is on old, low-metallicity GCs, our $\texttt{CMC}$ simulations follow the evolution of clusters over a Hubble time, and they include a wide range of metallicities (up to solar), so that our results can also be used to study younger and higher-metallicity star clusters.

==> other_figures.tex <==
\section{Radial Profiles}

\section{Stellar populations over time}

Recreate Nbh vs time plot from Section 3.2 for all other stellar populations.

\section{Lagrange radii}

\section{Mass segregation}
Newlin will make these plots.

\section{Overview of \texttt{CMC} output files}

\newpage

\newpage

\startlongtable
\begin{deluxetable*}{l|c|c|c|c||ccccc|cccc|ccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Stellar Mergers \label{table:models}}
\tablehead{
	\colhead{Model} &
    \colhead{$N$}&
    \colhead{$r_v$}&
    \colhead{$R_{\rm{gc}}$}&
    \colhead{$Z$}&
    \colhead{MS-MS}&
    \colhead{MS-G}&
    \colhead{MS-WD}&
    \colhead{MS-NS}&
    \colhead{MS-BH}&
    \colhead{G-G}&
    \colhead{G-WD}&
    \colhead{G-NS}&
    \colhead{G-BH}&
    \colhead{WD-WD}&
    \colhead{WD-NS}&
    \colhead{WD-BH}\\
    \colhead{}&
    \colhead{$\times10^5$}&
    \colhead{pc}&
    \colhead{kpc}&
    \colhead{$Z_{\odot}$}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}
}
\startdata
1 & 2 & 0.5 & 2 & 0.01 & 39 & 444 & 3 & 0 & 1 & 27 & 24 & 0 & 3 & 7 & 0 & 0 \\
2 & 4 & 0.5 & 2 & 0.01 & 132 & 903 & 0 & 0 & 14 & 28 & 59 & 0 & 1 & 11 & 3 & 0 \\
3 & 8 & 0.5 & 2 & 0.01 & 1393 & 3610 & 25 & 0 & 1 & 60 & 236 & 13 & 1 & 86 & 12 & 7 \\
4 & 16 & 0.5 & 2 & 0.01 & - & - & - & - & - & - & - & - & - & - & - & -  \\
\hline
5 & 2 & 0.5 & 2 & 0.1 & 70 & 691 & 0 & 0 & 1 & 23 & 22 & 0 & 1 & 15 & 0 & 1 \\
6 & 4 & 0.5 & 2 & 0.1 & 359 & 1664 & 5 & 0 & 2 & 15 & 90 & 4 & 2 & 29 & 1 & 1 \\
7 & 8 & 0.5 & 2 & 0.1 & 1666 & 3597 & 12 & 0 & 1 & 53 & 252 & 10 & 1 & 65 & 15 & 2 \\
8 & 16 & 0.5 & 2 & 0.1 & 5348 & 7544 & 22 & 0 & 0 & 64 & 337 & 14 & 0 & 89 & 0 & 1 \\
\hline
9 & 2 & 0.5 & 2 & 1.0 & 91 & 503 & 0 & 0 & 0 & 11 & 17 & 4 & 0 & 3 & 0 & 0 \\
10 & 4 & 0.5 & 2 & 1.0 & 455 & 1103 & 11 & 1 & 1 & 51 & 89 & 7 & 0 & 5 & 0 & 0 \\
11 & 8 & 0.5 & 2 & 1.0 & 1849 & 2206 & 12 & 1 & 0 & 73 & 190 & 16 & 2 & 58 & 0 & 1 \\
12 & 16 & 0.5 & 2 & 1.0 & 5564 & 4590 & 20 & 0 & 0 & 86 & 317 & 29 & 3 & 82 & 11 & 2 \\
\hline
13 & 2 & 0.5 & 8 & 0.01 & 60 & 677 & 0 & 0 & 16 & 16 & 13 & 0 & 0 & 8 & 0 & 0 \\
14 & 4 & 0.5 & 8 & 0.01 & 334 & 1769 & 6 & 0 & 9 & 25 & 117 & 2 & 0 & 42 & 2 & 1 \\
15 & 8 & 0.5 & 8 & 0.01 & 1674 & 3751 & 21 & 0 & 1 & 53 & 224 & 9 & 1 & 82 & 27 & 7 \\
16 & 16 & 0.5 & 8 & 0.01 & - & - & - & - & - & - & - & - & - & - & - & -  \\
\hline
17 & 2 & 0.5 & 8 & 0.1 & 153 & 781 & 6 & 0 & 0 & 32 & 51 & 0 & 0 & 20 & 0 & 1 \\
18 & 4 & 0.5 & 8 & 0.1 & 661 & 1837 & 4 & 0 & 0 & 23 & 119 & 4 & 1 & 42 & 2 & 1 \\
19 & 8 & 0.5 & 8 & 0.1 & 1925 & 3936 & 16 & 0 & 2 & 53 & 212 & 10 & 0 & 61 & 5 & 4 \\
20 & 16 & 0.5 & 8 & 0.1 & 5751 & 7685 & 21 & 0 & 1 & 71 & 335 & 16 & 0 & 74 & 1 & 0 \\
\hline
21 & 2 & 0.5 & 8 & 1.0 & 159 & 544 & 7 & 1 & 0 & 21 & 30 & 1 & 0 & 4 & 0 & 0 \\
22 & 4 & 0.5 & 8 & 1.0 & 636 & 1225 & 25 & 3 & 0 & 45 & 42 & 1 & 0 & 11 & 0 & 1 \\
23 & 8 & 0.5 & 8 & 1.0 & 2031 & 2270 & 35 & 8 & 0 & 65 & 161 & 7 & 4 & 17 & 0 & 5 \\
24 & 16 & 0.5 & 8 & 1.0 & 6037 & 4750 & 22 & 1 & 0 & 51 & 316 & 24 & 6 & 78 & 7 & 2 \\
\hline
25 & 2 & 0.5 & 20 & 0.01 & 127 & 651 & 14 & 0 & 3 & 35 & 41 & 0 & 0 & 20 & 1 & 0 \\
26 & 4 & 0.5 & 20 & 0.01 & 517 & 1801 & 6 & 0 & 2 & 17 & 68 & 1 & 5 & 30 & 0 & 19 \\
27 & 8 & 0.5 & 20 & 0.01 & 1805 & 4049 & 31 & 0 & 1 & 57 & 215 & 9 & 1 & 79 & 19 & 2 \\
28 & 16 & 0.5 & 20 & 0.01 & - & - & - & - & - & - & - & - & - & - & - & -  \\
\hline
29 & 2 & 0.5 & 20 & 0.1 & 178 & 904 & 5 & 0 & 0 & 24 & 43 & 0 & 1 & 21 & 0 & 0 \\
30 & 4 & 0.5 & 20 & 0.1 & 684 & 1820 & 8 & 0 & 1 & 28 & 103 & 2 & 0 & 30 & 2 & 1 \\
31 & 8 & 0.5 & 20 & 0.1 & 2072 & 3863 & 12 & 0 & 0 & 48 & 202 & 4 & 3 & 48 & 4 & 3 \\
32 & 16 & 0.5 & 20 & 0.1 & 5940 & 7618 & 21 & 0 & 1 & 65 & 324 & 3 & 0 & 90 & 2 & 0 \\
\hline
33 & 2 & 0.5 & 20 & 1.0 & 246 & 590 & 6 & 1 & 0 & 22 & 38 & 1 & 0 & 5 & 0 & 0 \\
34 & 4 & 0.5 & 20 & 1.0 & 859 & 1214 & 18 & 2 & 0 & 46 & 62 & 2 & 1 & 8 & 0 & 1 \\
35 & 8 & 0.5 & 20 & 1.0 & 2250 & 2309 & 10 & 1 & 2 & 51 & 159 & 13 & 1 & 36 & 1 & 3 \\
36 & 16 & 0.5 & 20 & 1.0 & 6199 & 4637 & 25 & 5 & 0 & 103 & 380 & 25 & 6 & 53 & 10 & 7 \\
\hline
37 & 2 & 1 & 2 & 0.01 & 12 & 632 & 23 & 0 & 0 & 18 & 46 & 1 & 0 & 30 & 0 & 0 \\
38 & 4 & 1 & 2 & 0.01 & 36 & 1823 & 52 & 0 & 1 & 19 & 107 & 2 & 5 & 51 & 4 & 0 \\
39 & 8 & 1 & 2 & 0.01 & 117 & 4086 & 77 & 0 & 1 & 52 & 141 & 2 & 3 & 42 & 0 & 1 \\
40 & 16 & 1 & 2 & 0.01 & 389 & 8114 & 95 & 0 & 2 & 100 & 256 & 3 & 0 & 73 & 0 & 0 \\
\hline
41 & 2 & 1 & 2 & 0.1 & 26 & 706 & 11 & 0 & 4 & 17 & 42 & 4 & 2 & 13 & 0 & 0 \\
42 & 4 & 1 & 2 & 0.1 & 56 & 1793 & 38 & 0 & 5 & 25 & 118 & 7 & 1 & 36 & 0 & 0 \\
43 & 8 & 1 & 2 & 0.1 & 100 & 4075 & 43 & 0 & 11 & 49 & 170 & 17 & 2 & 51 & 0 & 0 \\
44 & 16 & 1 & 2 & 0.1 & - & - & - & - & - & - & - & - & - & - & - & -  \\
\hline
45 & 2 & 1 & 2 & 1.0 & 68 & 546 & 29 & 3 & 0 & 19 & 26 & 0 & 0 & 7 & 0 & 0 \\
46 & 4 & 1 & 2 & 1.0 & 135 & 1405 & 59 & 8 & 1 & 38 & 70 & 1 & 3 & 19 & 1 & 6 \\
47 & 8 & 1 & 2 & 1.0 & 304 & 3021 & 144 & 13 & 2 & 85 & 111 & 0 & 1 & 29 & 0 & 1 \\
48 & 16 & 1 & 2 & 1.0 & 747 & 6188 & 225 & 22 & 14 & 221 & 279 & 2 & 0 & 39 & 0 & 0 \\
\hline
49 & 2 & 1 & 8 & 0.01 & 23 & 696 & 24 & 0 & 0 & 20 & 42 & 4 & 1 & 35 & 0 & 0 \\
50 & 4 & 1 & 8 & 0.01 & 60 & 1888 & 74 & 0 & 0 & 28 & 99 & 1 & 1 & 44 & 1 & 8 \\
51 & 8 & 1 & 8 & 0.01 & 117 & 4272 & 73 & 0 & 0 & 52 & 143 & 3 & 6 & 40 & 0 & 0 \\
52 & 16 & 1 & 8 & 0.01 & 450 & 8736 & 108 & 0 & 2 & 79 & 272 & 8 & 16 & 70 & 0 & 0 \\
\hline
53 & 2 & 1 & 8 & 0.1 & 22 & 787 & 22 & 0 & 2 & 13 & 53 & 2 & 1 & 12 & 0 & 4 \\
54 & 4 & 1 & 8 & 0.1 & 45 & 1978 & 52 & 0 & 5 & 22 & 79 & 8 & 1 & 29 & 1 & 1 \\
55 & 8 & 1 & 8 & 0.1 & 104 & 4159 & 39 & 1 & 8 & 52 & 202 & 21 & 5 & 39 & 0 & 0 \\
56 & 16 & 1 & 8 & 0.1 & - & - & - & - & - & - & - & - & - & - & - & -  \\
\hline
57 & 2 & 1 & 8 & 1.0 & 61 & 640 & 27 & 0 & 2 & 14 & 38 & 1 & 0 & 6 & 0 & 3 \\
58 & 4 & 1 & 8 & 1.0 & 116 & 1437 & 59 & 8 & 4 & 42 & 69 & 1 & 1 & 20 & 0 & 1 \\
59 & 8 & 1 & 8 & 1.0 & 294 & 3102 & 146 & 13 & 4 & 84 & 127 & 1 & 0 & 21 & 1 & 1 \\
60 & 16 & 1 & 8 & 1.0 & 750 & 6118 & 275 & 29 & 14 & 189 & 217 & 1 & 2 & 38 & 0 & 2 \\
\hline
61 & 2 & 1 & 20 & 0.01 & 14 & 735 & 37 & 0 & 0 & 19 & 44 & 0 & 3 & 46 & 2 & 0 \\
62 & 4 & 1 & 20 & 0.01 & - & - & - & - & - & - & - & - & - & - & - & -  \\
63 & 8 & 1 & 20 & 0.01 & 119 & 4298 & 77 & 0 & 1 & 51 & 141 & 4 & 3 & 37 & 0 & 0 \\
64 & 16 & 1 & 20 & 0.01 & 477 & 8804 & 108 & 0 & 1 & 77 & 270 & 7 & 19 & 72 & 0 & 0 \\
\hline
65 & 2 & 1 & 20 & 0.1 & 27 & 738 & 21 & 0 & 1 & 11 & 47 & 4 & 3 & 19 & 0 & 5 \\
66 & 4 & 1 & 20 & 0.1 & 50 & 1991 & 45 & 0 & 2 & 21 & 103 & 5 & 2 & 32 & 0 & 0 \\
67 & 8 & 1 & 20 & 0.1 & 90 & 4228 & 49 & 1 & 3 & 45 & 173 & 19 & 3 & 43 & 1 & 0 \\
68 & 16 & 1 & 20 & 0.1 & 208 & 8803 & 76 & 1 & 22 & 70 & 349 & 36 & 4 & 99 & 1 & 0 \\
\hline
69 & 2 & 1 & 20 & 1.0 & 63 & 600 & 28 & 2 & 0 & 17 & 37 & 0 & 0 & 15 & 0 & 2 \\
70 & 4 & 1 & 20 & 1.0 & 126 & 1456 & 51 & 10 & 4 & 34 & 65 & 0 & 1 & 27 & 0 & 0 \\
71 & 8 & 1 & 20 & 1.0 & 314 & 3109 & 154 & 19 & 6 & 71 & 102 & 0 & 0 & 21 & 0 & 1 \\
72 & 16 & 1 & 20 & 1.0 & 649 & 6370 & 33 & 19 & 11 & 172 & 412 & 16 & 0 & 68 & 0 & 1 \\
\hline
73 & 2 & 2 & 2 & 0.01 & 3 & 423 & 26 & 0 & 2 & 19 & 29 & 1 & 1 & 46 & 0 & 3 \\
74 & 4 & 2 & 2 & 0.01 & 11 & 1285 & 152 & 0 & 1 & 21 & 87 & 6 & 6 & 88 & 0 & 0 \\
75 & 8 & 2 & 2 & 0.01 & 30 & 3265 & 296 & 0 & 3 & 51 & 150 & 5 & 10 & 77 & 0 & 1 \\
76 & 16 & 2 & 2 & 0.01 & 64 & 7610 & 419 & 0 & 8 & 75 & 280 & 15 & 31 & 106 & 0 & 0 \\
\hline
77 & 2 & 2 & 2 & 0.1 & 15 & 496 & 21 & 0 & 1 & 20 & 53 & 4 & 0 & 25 & 0 & 0 \\
78 & 4 & 2 & 2 & 0.1 & 37 & 1409 & 102 & 0 & 6 & 22 & 103 & 8 & 0 & 39 & 0 & 1 \\
79 & 8 & 2 & 2 & 0.1 & 85 & 3375 & 172 & 0 & 13 & 51 & 197 & 17 & 0 & 52 & 0 & 0 \\
80 & 16 & 2 & 2 & 0.1 & 172 & 7683 & 222 & 0 & 45 & 85 & 403 & 24 & 5 & 108 & 1 & 0 \\
\hline
81 & 2 & 2 & 2 & 1.0 & 60 & 449 & 37 & 2 & 2 & 13 & 36 & 0 & 0 & 9 & 0 & 0 \\
82 & 4 & 2 & 2 & 1.0 & 125 & 1283 & 95 & 9 & 3 & 22 & 74 & 0 & 2 & 11 & 0 & 0 \\
83 & 8 & 2 & 2 & 1.0 & 292 & 2794 & 166 & 15 & 11 & 78 & 153 & 0 & 3 & 19 & 0 & 0 \\
84 & 16 & 2 & 2 & 1.0 & 426 & 6102 & 304 & 22 & 20 & 184 & 337 & 2 & 4 & 22 & 0 & 0 \\
\hline
85 & 2 & 2 & 8 & 0.01 & 5 & 523 & 89 & 0 & 0 & 23 & 27 & 0 & 1 & 68 & 0 & 0 \\
86 & 4 & 2 & 8 & 0.01 & - & - & - & - & - & - & - & - & - & - & - & -  \\
87 & 8 & 2 & 8 & 0.01 & 27 & 3400 & 328 & 0 & 1 & 52 & 149 & 4 & 8 & 75 & 0 & 0 \\
88 & 16 & 2 & 8 & 0.01 & 60 & 7899 & 443 & 0 & 14 & 80 & 270 & 18 & 29 & 107 & 0 & 0 \\
\hline
89 & 2 & 2 & 8 & 0.1 & 16 & 594 & 63 & 0 & 0 & 18 & 62 & 1 & 0 & 31 & 0 & 0 \\
90 & 4 & 2 & 8 & 0.1 & 42 & 1476 & 118 & 0 & 5 & 23 & 109 & 5 & 1 & 36 & 1 & 0 \\
91 & 8 & 2 & 8 & 0.1 & 91 & 3505 & 187 & 0 & 16 & 49 & 193 & 17 & 2 & 77 & 0 & 0 \\
92 & 16 & 2 & 8 & 0.1 & 143 & 7902 & 249 & 0 & 43 & 81 & 390 & 28 & 2 & 121 & 0 & 0 \\
\hline
93 & 2 & 2 & 8 & 1.0 & 68 & 531 & 49 & 3 & 1 & 18 & 41 & 0 & 0 & 14 & 0 & 0 \\
94 & 4 & 2 & 8 & 1.0 & 120 & 1308 & 109 & 8 & 6 & 20 & 68 & 0 & 1 & 14 & 0 & 0 \\
95 & 8 & 2 & 8 & 1.0 & 274 & 2837 & 159 & 13 & 13 & 76 & 151 & 0 & 3 & 22 & 0 & 0 \\
96 & 16 & 2 & 8 & 1.0 & 465 & 6079 & 301 & 30 & 19 & 190 & 327 & 1 & 8 & 29 & 0 & 0 \\
\hline
97 & 2 & 2 & 20 & 0.01 & 6 & 548 & 84 & 0 & 2 & 20 & 33 & 1 & 1 & 62 & 0 & 0 \\
98 & 4 & 2 & 20 & 0.01 & 18 & 1397 & 194 & 0 & 0 & 21 & 82 & 2 & 5 & 83 & 0 & 0 \\
99 & 8 & 2 & 20 & 0.01 & 32 & 3426 & 334 & 0 & 3 & 58 & 138 & 5 & 7 & 79 & 0 & 0 \\
100 & 16 & 2 & 20 & 0.01 & 72 & 7940 & 464 & 0 & 13 & 76 & 281 & 15 & 26 & 107 & 0 & 0 \\
\hline
101 & 2 & 2 & 20 & 0.1 & 22 & 593 & 71 & 0 & 2 & 16 & 58 & 1 & 0 & 27 & 0 & 0 \\
102 & 4 & 2 & 20 & 0.1 & 34 & 1506 & 114 & 0 & 6 & 27 & 112 & 6 & 0 & 37 & 0 & 0 \\
103 & 8 & 2 & 20 & 0.1 & 77 & 3544 & 196 & 0 & 14 & 57 & 201 & 18 & 0 & 58 & 0 & 0 \\
104 & 16 & 2 & 20 & 0.1 & 168 & 7879 & 246 & 1 & 45 & 72 & 415 & 28 & 4 & 121 & 0 & 1 \\
\hline
105 & 2 & 2 & 20 & 1.0 & 67 & 518 & 54 & 2 & 0 & 13 & 43 & 1 & 1 & 12 & 0 & 0 \\
106 & 4 & 2 & 20 & 1.0 & 147 & 1314 & 106 & 6 & 3 & 19 & 79 & 1 & 2 & 9 & 0 & 0 \\
107 & 8 & 2 & 20 & 1.0 & 265 & 2856 & 152 & 16 & 11 & 78 & 160 & 0 & 3 & 14 & 0 & 0 \\
108 & 16 & 2 & 20 & 1.0 & 405 & 6186 & 300 & 25 & 16 & 182 & 342 & 0 & 3 & 29 & 0 & 0 \\
\hline
109 & 2 & 4 & 2 & 0.01 & 5 & 124 & 0 & 0 & 0 & 21 & 34 & 0 & 0 & 15 & 0 & 0 \\
110 & 4 & 4 & 2 & 0.01 & 22 & 403 & 26 & 0 & 0 & 38 & 95 & 1 & 3 & 116 & 0 & 0 \\
111 & 8 & 4 & 2 & 0.01 & 51 & 1256 & 178 & 0 & 1 & 91 & 181 & 4 & 2 & 264 & 0 & 0 \\
112 & 16 & 4 & 2 & 0.01 & 106 & 3589 & 1009 & 0 & 2 & 113 & 288 & 5 & 10 & 413 & 0 & 0 \\
\hline
113 & 2 & 4 & 2 & 0.1 & 16 & 156 & 4 & 0 & 1 & 27 & 37 & 1 & 0 & 27 & 0 & 0 \\
114 & 4 & 4 & 2 & 0.1 & 45 & 510 & 35 & 1 & 2 & 32 & 137 & 4 & 0 & 58 & 0 & 0 \\
115 & 8 & 4 & 2 & 0.1 & 110 & 1549 & 186 & 3 & 4 & 84 & 244 & 18 & 1 & 117 & 0 & 0 \\
116 & 16 & 4 & 2 & 0.1 & 167 & 4434 & 839 & 1 & 8 & 143 & 375 & 38 & 12 & 276 & 0 & 0 \\
\hline
117 & 2 & 4 & 2 & 1.0 & 98 & 146 & 37 & 3 & 0 & 14 & 33 & 0 & 0 & 13 & 0 & 0 \\
118 & 4 & 4 & 2 & 1.0 & 241 & 506 & 116 & 4 & 1 & 14 & 67 & 0 & 0 & 17 & 0 & 0 \\
119 & 8 & 4 & 2 & 1.0 & 641 & 1437 & 386 & 3 & 1 & 12 & 97 & 0 & 0 & 13 & 0 & 0 \\
120 & 16 & 4 & 2 & 1.0 & 1281 & 3788 & 772 & 9 & 3 & 19 & 109 & 0 & 2 & 17 & 0 & 0 \\
\hline
121 & 2 & 4 & 8 & 0.01 & 4 & 185 & 61 & 0 & 0 & 25 & 41 & 0 & 0 & 115 & 0 & 1 \\
122 & 4 & 4 & 8 & 0.01 & 20 & 508 & 165 & 0 & 0 & 41 & 103 & 1 & 3 & 217 & 0 & 0 \\
123 & 8 & 4 & 8 & 0.01 & 37 & 1411 & 452 & 0 & 1 & 89 & 189 & 7 & 4 & 318 & 0 & 0 \\
124 & 16 & 4 & 8 & 0.01 & 103 & 3695 & 1185 & 0 & 6 & 122 & 288 & 7 & 10 & 436 & 0 & 0 \\
\hline
125 & 2 & 4 & 8 & 0.1 & 13 & 250 & 67 & 0 & 0 & 25 & 86 & 2 & 0 & 52 & 0 & 0 \\
126 & 4 & 4 & 8 & 0.1 & 35 & 652 & 163 & 2 & 2 & 37 & 179 & 4 & 2 & 73 & 0 & 0 \\
127 & 8 & 4 & 8 & 0.1 & 84 & 1749 & 403 & 1 & 3 & 82 & 259 & 15 & 2 & 131 & 0 & 0 \\
128 & 16 & 4 & 8 & 0.1 & 187 & 4518 & 938 & 3 & 11 & 155 & 372 & 41 & 9 & 262 & 0 & 0 \\
\hline
129 & 2 & 4 & 8 & 1.0 & 94 & 221 & 86 & 1 & 0 & 13 & 55 & 0 & 0 & 24 & 0 & 0 \\
130 & 4 & 4 & 8 & 1.0 & 283 & 565 & 206 & 3 & 2 & 17 & 79 & 0 & 1 & 20 & 0 & 0 \\
131 & 8 & 4 & 8 & 1.0 & 613 & 1516 & 420 & 3 & 3 & 12 & 101 & 1 & 0 & 15 & 0 & 0 \\
132 & 16 & 4 & 8 & 1.0 & 1268 & 3856 & 783 & 16 & 4 & 19 & 104 & 0 & 1 & 25 & 0 & 0 \\
\hline
133 & 2 & 4 & 20 & 0.01 & 5 & 188 & 75 & 0 & 1 & 23 & 48 & 1 & 1 & 124 & 0 & 0 \\
134 & 4 & 4 & 20 & 0.01 & 22 & 508 & 162 & 0 & 1 & 45 & 105 & 1 & 0 & 220 & 0 & 0 \\
135 & 8 & 4 & 20 & 0.01 & 38 & 1406 & 468 & 0 & 1 & 94 & 182 & 5 & 3 & 327 & 0 & 0 \\
136 & 16 & 4 & 20 & 0.01 & 112 & 3690 & 1204 & 0 & 2 & 121 & 296 & 9 & 16 & 422 & 0 & 0 \\
\hline
137 & 2 & 4 & 20 & 0.1 & 14 & 249 & 69 & 0 & 0 & 25 & 81 & 2 & 0 & 53 & 0 & 0 \\
138 & 4 & 4 & 20 & 0.1 & 32 & 665 & 168 & 3 & 0 & 35 & 182 & 4 & 0 & 75 & 0 & 0 \\
139 & 8 & 4 & 20 & 0.1 & 92 & 1770 & 419 & 0 & 1 & 87 & 268 & 14 & 3 & 118 & 0 & 0 \\
140 & 16 & 4 & 20 & 0.1 & 208 & 4566 & 932 & 3 & 15 & 143 & 374 & 36 & 9 & 266 & 0 & 0 \\
\hline
141 & 2 & 4 & 20 & 1.0 & 92 & 222 & 86 & 2 & 1 & 14 & 58 & 0 & 0 & 25 & 0 & 0 \\
142 & 4 & 4 & 20 & 1.0 & 260 & 596 & 197 & 2 & 1 & 16 & 76 & 0 & 1 & 24 & 0 & 0 \\
143 & 8 & 4 & 20 & 1.0 & 628 & 1508 & 413 & 4 & 1 & 13 & 98 & 0 & 0 & 15 & 0 & 0 \\
144 & 16 & 4 & 20 & 1.0 & 1279 & 3853 & 778 & 12 & 4 & 18 & 101 & 1 & 1 & 25 & 0 & 0 \\
\enddata
\tablecomments{}
\end{deluxetable*}


\startlongtable
\begin{deluxetable*}{l|c|c|c|cccccc|c}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{BBH mergers for all model GCs\label{table:models}}
\tablehead{
	\colhead{Model} &
    \colhead{$N$}&
    \colhead{$r_v$}&
    \colhead{$R_{\rm{gc}}$}&
    \colhead{$Z$}&
    \colhead{$N_{\rm{BH}}$ at 12 Gyr}&
    \colhead{FB-capture}&
    \colhead{SS-capture}&
    \colhead{In-cluster}&
    \colhead{Ejected}&
    \colhead{Total}\\
    \colhead{}&
    \colhead{$\times10^5$}&
    \colhead{pc}&
    \colhead{kpc}&
    \colhead{$Z_{\odot}$}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}&
    \colhead{}
}
\startdata
1 & 2 & 0.5 & 2 & 0.01 & - & 4 & 0 & 5 & 12 & 21 \\
2 & 4 & 0.5 & 2 & 0.01 & - & 9 & 1 & 16 & 42 & 68 \\
3 & 8 & 0.5 & 2 & 0.01 & 0 & 26 & 3 & 45 & 0 & 74 \\
4 & 16 & 0.5 & 2 & 0.01 & - & - & - & - & - & -  \\
\hline
5 & 2 & 0.5 & 2 & 0.1 & - & 7 & 0 & 2 & 9 & 18 \\
6 & 4 & 0.5 & 2 & 0.1 & - & 5 & 0 & 11 & 28 & 44 \\
7 & 8 & 0.5 & 2 & 0.1 & 0 & 16 & 2 & 44 & 72 & 134 \\
8 & 16 & 0.5 & 2 & 0.1 & 53 & 46 & 13 & 151 & 163 & 373 \\
\hline
9 & 2 & 0.5 & 2 & 1.0 & - & 3 & 0 & 3 & 8 & 14 \\
10 & 4 & 0.5 & 2 & 1.0 & - & 3 & 1 & 9 & 17 & 30 \\
11 & 8 & 0.5 & 2 & 1.0 & 0 & 18 & 0 & 48 & 55 & 121 \\
12 & 16 & 0.5 & 2 & 1.0 & 1 & 28 & 13 & 183 & 140 & 364 \\
\hline
13 & 2 & 0.5 & 8 & 0.01 & - & 5 & 0 & 4 & 14 & 23 \\
14 & 4 & 0.5 & 8 & 0.01 & 0 & 14 & 0 & 20 & 39 & 73 \\
15 & 8 & 0.5 & 8 & 0.01 & 0 & 25 & 0 & 49 & 80 & 154 \\
16 & 16 & 0.5 & 8 & 0.01 & - & - & - & - & - & -  \\
\hline
17 & 2 & 0.5 & 8 & 0.1 & 0 & 5 & 0 & 3 & 8 & 16 \\
18 & 4 & 0.5 & 8 & 0.1 & 0 & 7 & 2 & 15 & 38 & 62 \\
19 & 8 & 0.5 & 8 & 0.1 & 1 & 17 & 1 & 42 & 82 & 142 \\
20 & 16 & 0.5 & 8 & 0.1 & 69 & 49 & 11 & 134 & 178 & 372 \\
\hline
21 & 2 & 0.5 & 8 & 1.0 & 0 & 0 & 0 & 3 & 10 & 13 \\
22 & 4 & 0.5 & 8 & 1.0 & - & 2 & 0 & 6 & 26 & 34 \\
23 & 8 & 0.5 & 8 & 1.0 & 1 & 7 & 2 & 61 & 57 & 127 \\
24 & 16 & 0.5 & 8 & 1.0 & 6 & 39 & 19 & 201 & 136 & 395 \\
\hline
25 & 2 & 0.5 & 20 & 0.01 & 0 & 2 & 0 & 9 & 13 & 24 \\
26 & 4 & 0.5 & 20 & 0.01 & 1 & 9 & 0 & 13 & 37 & 59 \\
27 & 8 & 0.5 & 20 & 0.01 & 1 & 19 & 2 & 47 & 84 & 152 \\
28 & 16 & 0.5 & 20 & 0.01 & - & - & - & - & - & -  \\
\hline
29 & 2 & 0.5 & 20 & 0.1 & 0 & 6 & 0 & 5 & 10 & 21 \\
30 & 4 & 0.5 & 20 & 0.1 & 0 & 7 & 0 & 23 & 25 & 55 \\
31 & 8 & 0.5 & 20 & 0.1 & 7 & 18 & 4 & 52 & 77 & 151 \\
32 & 16 & 0.5 & 20 & 0.1 & 92 & 58 & 13 & 156 & 167 & 394 \\
\hline
33 & 2 & 0.5 & 20 & 1.0 & 0 & 1 & 0 & 2 & 6 & 9 \\
34 & 4 & 0.5 & 20 & 1.0 & 0 & 8 & 0 & 18 & 14 & 40 \\
35 & 8 & 0.5 & 20 & 1.0 & 4 & 9 & 0 & 52 & 60 & 121 \\
36 & 16 & 0.5 & 20 & 1.0 & 5 & 40 & 13 & 198 & 126 & 377 \\
\hline
37 & 2 & 1 & 2 & 0.01 & - & 6 & 0 & 6 & 3 & 15 \\
38 & 4 & 1 & 2 & 0.01 & 0 & 5 & 0 & 9 & 18 & 32 \\
39 & 8 & 1 & 2 & 0.01 & 11 & 19 & 3 & 32 & 57 & 111 \\
40 & 16 & 1 & 2 & 0.01 & 199 & 51 & 14 & 104 & 134 & 303 \\
\hline
41 & 2 & 1 & 2 & 0.1 & - & 3 & 0 & 1 & 5 & 9 \\
42 & 4 & 1 & 2 & 0.1 & 0 & 5 & 1 & 11 & 18 & 35 \\
43 & 8 & 1 & 2 & 0.1 & 28 & 20 & 3 & 34 & 42 & 99 \\
44 & 16 & 1 & 2 & 0.1 & - & 21 & 8 & 92 & 130 & 251 \\
\hline
45 & 2 & 1 & 2 & 1.0 & - & 4 & 0 & 5 & 5 & 14 \\
46 & 4 & 1 & 2 & 1.0 & 1 & 4 & 0 & 8 & 9 & 21 \\
47 & 8 & 1 & 2 & 1.0 & 10 & 7 & 0 & 39 & 54 & 100 \\
48 & 16 & 1 & 2 & 1.0 & 131 & 15 & 9 & 123 & 120 & 267 \\
\hline
49 & 2 & 1 & 8 & 0.01 & 0 & 1 & 0 & 3 & 3 & 7 \\
50 & 4 & 1 & 8 & 0.01 & 1 & 8 & 1 & 10 & 29 & 48 \\
51 & 8 & 1 & 8 & 0.01 & 34 & 15 & 0 & 31 & 61 & 107 \\
52 & 16 & 1 & 8 & 0.01 & 240 & 41 & 16 & 100 & 143 & 300 \\
\hline
53 & 2 & 1 & 8 & 0.1 & 0 & 6 & 0 & 2 & 9 & 17 \\
54 & 4 & 1 & 8 & 0.1 & 1 & 8 & 0 & 7 & 21 & 36 \\
55 & 8 & 1 & 8 & 0.1 & 31 & 12 & 3 & 41 & 58 & 114 \\
56 & 16 & 1 & 8 & 0.1 & 227 & 39 & 7 & 121 & 140 & 307 \\
\hline
57 & 2 & 1 & 8 & 1.0 & 0 & 1 & 0 & 3 & 7 & 11 \\
58 & 4 & 1 & 8 & 1.0 & 0 & 7 & 1 & 12 & 18 & 38 \\
59 & 8 & 1 & 8 & 1.0 & 19 & 7 & 3 & 47 & 41 & 98 \\
60 & 16 & 1 & 8 & 1.0 & 143 & 26 & 7 & 122 & 116 & 271 \\
\hline
61 & 2 & 1 & 20 & 0.01 & 0 & 2 & 0 & 4 & 5 & 11 \\
62 & 4 & 1 & 20 & 0.01 & 0 & 1 & 0 & 6 & 31 & 38 \\
63 & 8 & 1 & 20 & 0.01 & 35 & 21 & 1 & 38 & 55 & 115 \\
64 & 16 & 1 & 20 & 0.01 & 250 & 39 & 11 & 106 & 145 & 301 \\
\hline
65 & 2 & 1 & 20 & 0.1 & 1 & 4 & 2 & 3 & 9 & 18 \\
66 & 4 & 1 & 20 & 0.1 & 3 & 5 & 1 & 12 & 24 & 42 \\
67 & 8 & 1 & 20 & 0.1 & 43 & 18 & 3 & 34 & 50 & 105 \\
68 & 16 & 1 & 20 & 0.1 & 257 & 32 & 12 & 100 & 139 & 283 \\
\hline
69 & 2 & 1 & 20 & 1.0 & 1 & 2 & 0 & 6 & 3 & 11 \\
70 & 4 & 1 & 20 & 1.0 & 3 & 2 & 0 & 9 & 12 & 23 \\
71 & 8 & 1 & 20 & 1.0 & 23 & 9 & 1 & 44 & 50 & 104 \\
72 & 16 & 1 & 20 & 1.0 & 154 & 19 & 8 & 129 & 116 & 272 \\
\hline
73 & 2 & 2 & 2 & 0.01 & - & 1 & 0 & 3 & 6 & 10 \\
74 & 4 & 2 & 2 & 0.01 & 2 & 7 & 0 & 6 & 17 & 30 \\
75 & 8 & 2 & 2 & 0.01 & 73 & 7 & 1 & 23 & 31 & 62 \\
76 & 16 & 2 & 2 & 0.01 & 489 & 24 & 7 & 65 & 103 & 199 \\
\hline
77 & 2 & 2 & 2 & 0.1 & - & 1 & 0 & 0 & 5 & 6 \\
78 & 4 & 2 & 2 & 0.1 & 1 & 3 & 0 & 5 & 13 & 21 \\
79 & 8 & 2 & 2 & 0.1 & 95 & 7 & 2 & 21 & 29 & 59 \\
80 & 16 & 2 & 2 & 0.1 & 497 & 20 & 2 & 49 & 84 & 155 \\
\hline
81 & 2 & 2 & 2 & 1.0 & - & 0 & 0 & 2 & 2 & 4 \\
82 & 4 & 2 & 2 & 1.0 & 16 & 1 & 0 & 3 & 9 & 13 \\
83 & 8 & 2 & 2 & 1.0 & 116 & 2 & 2 & 19 & 34 & 57 \\
84 & 16 & 2 & 2 & 1.0 & 433 & 12 & 6 & 50 & 63 & 131 \\
\hline
85 & 2 & 2 & 8 & 0.01 & 0 & 1 & 0 & 4 & 5 & 10 \\
86 & 4 & 2 & 8 & 0.01 & 13 & 4 & 1 & 8 & 15 & 28 \\
87 & 8 & 2 & 8 & 0.01 & 112 & 15 & 3 & 24 & 29 & 71 \\
88 & 16 & 2 & 8 & 0.01 & 610 & 20 & 6 & 60 & 94 & 180 \\
\hline
89 & 2 & 2 & 8 & 0.1 & 0 & 0 & 0 & 2 & 4 & 6 \\
90 & 4 & 2 & 8 & 0.1 & 16 & 4 & 1 & 8 & 12 & 25 \\
91 & 8 & 2 & 8 & 0.1 & 116 & 11 & 0 & 21 & 32 & 64 \\
92 & 16 & 2 & 8 & 0.1 & 541 & 19 & 5 & 53 & 81 & 158 \\
\hline
93 & 2 & 2 & 8 & 1.0 & 9 & 0 & 1 & 4 & 2 & 7 \\
94 & 4 & 2 & 8 & 1.0 & 52 & 1 & 0 & 6 & 9 & 16 \\
95 & 8 & 2 & 8 & 1.0 & 152 & 8 & 2 & 18 & 27 & 55 \\
96 & 16 & 2 & 8 & 1.0 & 441 & 13 & 3 & 38 & 74 & 128 \\
\hline
97 & 2 & 2 & 20 & 0.01 & 3 & 2 & 0 & 1 & 4 & 7 \\
98 & 4 & 2 & 20 & 0.01 & 14 & 4 & 0 & 5 & 14 & 23 \\
99 & 8 & 2 & 20 & 0.01 & 117 & 8 & 1 & 23 & 36 & 68 \\
100 & 16 & 2 & 20 & 0.01 & 581 & 24 & 4 & 56 & 86 & 170 \\
\hline
101 & 2 & 2 & 20 & 0.1 & 3 & 1 & 0 & 1 & 3 & 5 \\
102 & 4 & 2 & 20 & 0.1 & 15 & 2 & 0 & 6 & 14 & 22 \\
103 & 8 & 2 & 20 & 0.1 & 142 & 7 & 2 & 18 & 29 & 56 \\
104 & 16 & 2 & 20 & 0.1 & 589 & 21 & 2 & 45 & 87 & 155 \\
\hline
105 & 2 & 2 & 20 & 1.0 & 7 & 0 & 0 & 2 & 1 & 3 \\
106 & 4 & 2 & 20 & 1.0 & 38 & 4 & 0 & 5 & 8 & 17 \\
107 & 8 & 2 & 20 & 1.0 & 151 & 5 & 1 & 16 & 22 & 44 \\
108 & 16 & 2 & 20 & 1.0 & 481 & 14 & 2 & 63 & 74 & 153 \\
\hline
109 & 2 & 4 & 2 & 0.01 & - & 0 & 0 & 3 & 3 & 6 \\
110 & 4 & 4 & 2 & 0.01 & - & 2 & 0 & 0 & 10 & 12 \\
111 & 8 & 4 & 2 & 0.01 & - & 1 & 0 & 6 & 17 & 24 \\
112 & 16 & 4 & 2 & 0.01 & 892 & 12 & 3 & 31 & -1 & 45 \\
\hline
113 & 2 & 4 & 2 & 0.1 & - & 0 & 0 & 1 & 4 & 5 \\
114 & 4 & 4 & 2 & 0.1 & - & 2 & 0 & 5 & 9 & 16 \\
115 & 8 & 4 & 2 & 0.1 & - & 5 & 0 & 5 & 24 & 34 \\
116 & 16 & 4 & 2 & 0.1 & 907 & 12 & 3 & 25 & 54 & 94 \\
\hline
117 & 2 & 4 & 2 & 1.0 & - & 0 & 0 & 0 & 2 & 2 \\
118 & 4 & 4 & 2 & 1.0 & - & 1 & 0 & 2 & 5 & 8 \\
119 & 8 & 4 & 2 & 1.0 & 300 & 3 & 0 & 6 & 17 & 26 \\
120 & 16 & 4 & 2 & 1.0 & 816 & 7 & 0 & 12 & 25 & 44 \\
\hline
121 & 2 & 4 & 8 & 0.01 & 6 & 0 & 0 & 3 & 3 & 6 \\
122 & 4 & 4 & 8 & 0.01 & 53 & 3 & 0 & 1 & 9 & 13 \\
123 & 8 & 4 & 8 & 0.01 & 330 & 11 & 0 & 9 & 20 & 40 \\
124 & 16 & 4 & 8 & 0.01 & 1090 & 8 & 2 & 28 & 44 & 82 \\
\hline
125 & 2 & 4 & 8 & 0.1 & 9 & 0 & 0 & 4 & 4 & 8 \\
126 & 4 & 4 & 8 & 0.1 & 68 & 1 & 0 & 1 & 11 & 13 \\
127 & 8 & 4 & 8 & 0.1 & 311 & 7 & 0 & 10 & 28 & 45 \\
128 & 16 & 4 & 8 & 0.1 & 989 & 9 & 5 & 37 & 49 & 100 \\
\hline
129 & 2 & 4 & 8 & 1.0 & 33 & 0 & 0 & 1 & 1 & 2 \\
130 & 4 & 4 & 8 & 1.0 & 133 & 2 & 1 & 2 & 5 & 10 \\
131 & 8 & 4 & 8 & 1.0 & 340 & 1 & 0 & 7 & 15 & 23 \\
132 & 16 & 4 & 8 & 1.0 & 834 & 7 & 0 & 25 & 27 & 59 \\
\hline
133 & 2 & 4 & 20 & 0.01 & 12 & 1 & 0 & 1 & 4 & 6 \\
134 & 4 & 4 & 20 & 0.01 & 68 & 2 & 0 & 2 & 10 & 14 \\
135 & 8 & 4 & 20 & 0.01 & 376 & 3 & 0 & 5 & 21 & 29 \\
136 & 16 & 4 & 20 & 0.01 & 1107 & 13 & 1 & 33 & 45 & 92 \\
\hline
137 & 2 & 4 & 20 & 0.1 & 11 & 1 & 0 & 2 & 5 & 8 \\
138 & 4 & 4 & 20 & 0.1 & 66 & 4 & 0 & 3 & 8 & 15 \\
139 & 8 & 4 & 20 & 0.1 & 327 & 2 & 1 & 15 & 21 & 39 \\
140 & 16 & 4 & 20 & 0.1 & 1026 & 11 & 3 & 31 & 52 & 97 \\
\hline
141 & 2 & 4 & 20 & 1.0 & 49 & 1 & 0 & 0 & 2 & 3 \\
142 & 4 & 4 & 20 & 1.0 & 125 & 3 & 0 & 1 & 6 & 10 \\
143 & 8 & 4 & 20 & 1.0 & 358 & 4 & 1 & 5 & 18 & 28 \\
144 & 16 & 4 & 20 & 1.0 & 856 & 6 & 1 & 15 & 28 & 50 \\
\enddata
\tablecomments{text...}
\end{deluxetable*}







\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{BBH_scatter}
\caption{\label{fig:BBH_scatter} Component masses for all BBH mergers. Black points mark first-generation mergers, green marks, 1.5-generation, and blue mark second-generation.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{radial_dist_2e5_002.pdf}
\caption{Cumulative radial distributions of all stellar populations (colors denoted in figure legend) for three cluster snapshots in time (from left to right, $t=$0.1, 1, and 10 Gyr). From top to bottom, we show clusters of varying initial virial radius, $r_v$. All initial other cluster parameters are fixed. The vertical dashed gray lines mark the core radius of each cluster snapshot. Note that models with smaller initial $r_v$ have fewer BHs and smaller core radii than large $r_v$ counterparts.} \label{fig:radial_dist_2e5_0.002}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{radial_dist_4e5_002.pdf}
\caption{Cumulative radial distributions of all stellar populations (colors denoted in figure legend) for three cluster snapshots in time (from left to right, $t=$0.1, 1, and 10 Gyr). From top to bottom, we show clusters of varying initial virial radius, $r_v$. All initial other cluster parameters are fixed. The vertical dashed gray lines mark the core radius of each cluster snapshot. Note that models with smaller initial $r_v$ have fewer BHs and smaller core radii than large $r_v$ counterparts.} \label{fig:radial_dist_4e5_0.002}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{radial_dist_16e6_002.pdf}
\caption{Cumulative radial distributions of all stellar populations (colors denoted in figure legend) for three cluster snapshots in time (from left to right, $t=$0.1, 1, and 10 Gyr). From top to bottom, we show clusters of varying initial virial radius, $r_v$. All initial other cluster parameters are fixed. The vertical dashed gray lines mark the core radius of each cluster snapshot. Note that models with smaller initial $r_v$ have fewer BHs and smaller core radii than large $r_v$ counterparts.} \label{fig:radial_dist_1.6e6_0.002}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{Nbbh_mergers}
\caption{\label{fig:BBHmergers} Number of BBH mergers of different classes, as described in the text. Darker to lighter shades of blue show larger to smaller initial $r_v$.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{BH_mf}
\caption{\label{fig:Mvsrcrh} Mass function for all BHs at birth (excluding second-generation BHs formed through BBH mergers). Here we show models with initial $N=8\times 10^5$.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{1G_mergers2}
\caption{\label{fig:Mvsrcrh} Component masses for all first-generation BHs that undergo mergers.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{2G_mergers2}
\caption{\label{fig:Mvsrcrh} Masses of all second-generation BHs that undergo mergers.}
\end{center}
\end{figure*}


\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{z001}
\caption{\label{fig:z001} \textit{Top row:} Lagrange radii for BH populations versus time for $0.01Z_{\odot}$ models with $N=8\times10^5$ and $r_{\rm{gc}}=8\,$kpc. $1\%,10\%,50\%,$ and $90\%$ Lagrange radii are shown in gray, black, blue, and red, respectively. \textit{Middle row:} Number density of the BHs for the same four percentiles versus time. \textit{Bottom row:} Total number of BHs versus time.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{z01}
\caption{\label{fig:z01} Same as Figure \ref{fig:z001} but for $0.1Z_{\odot}$ models.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{z1}
\caption{\label{fig:z1} Same as Figure \ref{fig:z001} but for $Z_{\odot}$ models.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{collisions}
\caption{\label{fig:collisions} Stellar collisions occurring through single--single encounters or during \texttt{fewbody} integrations of binary--single and binary--binary encounters.}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{mergers}
\caption{\label{fig:mergers} Stellar mergers occurring during binary evolution between dynamical encounters.}
\end{center}
\end{figure*}
